OptSmart: A Space Efficient Optimistic Concurrent Execution of Smart Contracts

Popular blockchains such as Ethereum and several others execute complex transactions in blocks through user-defined scripts known as smart contracts. Serial execution of smart contract transactions/atomic-units (AUs) fails to harness the multiprocessing power offered by the prevalence of multi-core processors. By adding concurrency to the execution of AUs, we can achieve better efficiency and higher throughput. In this paper, we develop a concurrent miner that proposes a block by executing the AUs concurrently using optimistic Software Transactional Memory systems (STMs). It captures the independent AUs in a concurrent bin and dependent AUs in the block graph (BG) efficiently. Later, we propose a concurrent validator that re-executes the same AUs concurrently and deterministically using a concurrent bin followed by a BG given by the miner to verify the proposed block. We rigorously prove the correctness of concurrent execution of AUs and achieve significant performance gain over the state-of-the-art.

==> authorBiography.tex <==
\newpage
\begin{center}
\textbf{\huge Author Biography}
\end{center}
%Author biography and role comes here....
\begin{figure}[H]
\includegraphics[width=0.25\textwidth, height=0.25\textwidth]{figs/authors/anjana.jpg}
\end{figure}
\noindent\textbf{Parwat Singh Anjana} is currently a doctoral student at the Department of Computer Science and Engineering at the Indian Institute of Technology Hyderabad, India. He received his M.Tech in Computer Science from the University of Hyderabad, India, in 2014. %He did his B.Tech in Computer Science and Engineering from Rajasthan Technical University, India, in 2011. 
His research interests include Blockchain Technology, Parallel and Distributed Computing, Software Transactional Memory, and Cloud Computing. 

\vspace{.25cm}
\begin{figure}[H]
\includegraphics[width=0.25\textwidth, height=0.25\textwidth]{figs/authors/sweta.jpg}
\end{figure}
\noindent\textbf{Sweta Kumari} is a Postdoctoral Scientist at the Department of Computer Science at the Technion Israel Institute of Technology working with Prof. Hagit Attiya. Her current research areas are Progress Guarantees in Transactional Memory Systems, Byzantine Tolerant in Dynamic Distributed System, Concurrent execution of Smart Contract in Blockchain, and Optimal resilience in the mixed model. She has completed her Ph.D. from the Department of CSE, IIT Hyderabad, in Feb 2020. %She did M.Tech from the Department of CSE, MANIT, Bhopal in 2014 and completed B.Tech in Information Technology from RCEW, Jaipur, Rajasthan in 2011.
\vspace{.25cm}
\begin{figure}[H]
\includegraphics[width=0.25\textwidth, height=0.25\textwidth]{figs/authors/sathya.png}
\end{figure}
\noindent\textbf{Dr. Sathya Peri} is currently an Associate Professor in the Department of Computer Science and Engineering at the Indian Institute of Technology Hyderabad (IITH), India. His research interests broadly comprise of parallel and distributed systems. In the context of distributed systems, his current research interest includes Blockchain and Peer-to-Peer Systems. He is currently working on improving the efficiency of Smart Contract Execution in Blockchains Systems.

\vspace{.25cm}
\begin{figure}[H]
\includegraphics[width=0.25\textwidth, height=0.25\textwidth]{figs/authors/sachin.jpg}
\end{figure}
\noindent\textbf{Sachin Rathor} is a masters student at IITH ....

\vspace{.25cm}
\begin{figure}[H]
\includegraphics[width=0.25\textwidth, height=0.25\textwidth]{figs/authors/archit1.jpg}
\end{figure}
\noindent\textbf{Archit Somain} is a Post-Doctoral Fellow at the Department of Computer Science at Technion, Israel Institute of Technology, working with Prof. Hagit Attiya. His research interests lie in Composable Concurrent Data Structures, Software Transactional Memory systems, Blockchain, Dynamic Distributed Algorithms, and Persistent Memory. He has completed his Ph.D. from the Department of CSE, IIT Hyderabad.% He earned M.Tech from the Department of CSE, MANIT, Bhopal in 2014 and a B.Tech in Information Technology from ITM, Bhilwara, Rajasthan in 2010.

==> cover.tex <==
\begin{center}
\textbf{\huge Cover Letter}
\end{center}

\noindent
\textbf{To:} JPDC Journal Editor and Reviewers\\
\textbf{Subject:} {\color{blue}Differences of submitted manuscript from conference version.}\\
%Differences from conference version to the submitted manuscript\\

\noindent
Dear Editor and Reviewers,\\

\noindent
We hope everything is fine with you, your family, and friends in the current COVID-19 pandemic.\\

\noindent

We are delighted to submit our extended paper title \emph{``OptSmart: A Space Efficient Optimistic Concurrent Execution of Smart Contracts"} in JPDC Journal. A preliminary version of this paper appeared in 27$^{th}$ Euromicro International Conference on Parallel, Distributed, and Network-Based Processing (PDP) 2019, Pavia, Italy. The differences of submitted manuscript from conference version are as follows:

\begin{itemize}
	\item We have included in-depth related work.
	\item We have explained the detailed description of our proposed mechanism. 
	\item We rigorously proved that the concurrent miner and validator satisfy correctness criterion as \emph{opacity}.
	\item We have proposed an \emph{efficient} and \emph{storage optimal} Block Graph approach that reduces the size of the block.
	%\item We have proposed an \emph{efficient} and \emph{storage optimal} Block Graph which in turn reduces the size of the block.
	\item It includes the exhaustive experiments comparison with state-of-the-art.
\end{itemize}

Thanks in advance for your time and effort to handle this paper.

\vspace{.5cm}
\noindent
Best regards,\\
Anjana et al.

==> highlights.tex <==
\begin{center}
\textbf{\huge Highlights}
\end{center}

\begin{itemize}
\item A novel approach to execute the \SContract{} transactions {\color{blue}(atomic-units)} by concurrent miner using \emph{optimistic} STMs, generic to any other STM protocol.

\item A \emph{lock-free} and concurrent graph library to generate the \emph{efficient} Block Graph which contains only dependent \au{s} and optimizes the size of the block in the state-of-the-art approaches.

\item A concurrent validator that re-executes the \SContract{} transactions deterministically and efficiently with the help of \emph{concurrent bin} followed by \emph{efficient} BG given by concurrent miner.

%\item For storage optimality and efficiency, we have optimized the size of the BG (see \secref{opt}). 


\item A rigorous proof that the concurrent miner {\color{blue}and validator} satisfies correctness criterion as \emph{opacity}. 

\item {\color{blue}Optimized concurrent miner} achieved {\color{red}4.10$\times$ and 4.55$\times$} average speedups using BTO and MVTO STM protocol, respectively. Optimized decentralized concurrent BTO and MVTO validator outperform average {\color{green}7.05$\times$ and 7.84$\times$} than serial validator, respectively.



%    \item A c

%    \item State-of-the-art approaches to estimate energy consumption in machine learning.

%    \item Software tools from the power and performance monitoring field and their applicability to machine learning.

%    \item Two use cases to estimate energy consumption for deep learning and data mining.
\end{itemize}

==> objective.tex <==
\vspace{-.1cm}
\section{Requirements of Concurrent Miner, Validator and Block Graph}
\label{sec:req-miner_val}

This section describes the requirements of concurrent miner, validator and block graph to ensure correct concurrent execution of the \scontract transactions. 

%\todo{In one of the sections below, bring the ideas of MVE, VE \& CE.}

\subsection{Requirements of the Concurrent Miner}
The miner process invokes several threads to concurrently execute the \scontract transactions or \au{s}. With the proposed optimistic execution approach, each miner thread invokes an \au as a transaction. %It is important to ensure that the concurrent execution is \emph{correct}. 

The miner should ensure the correct concurrent execution of the smart contract transactions. The incorrect concurrent execution (or consistency issues) may occur when concurrency involved. Any inconsistent read may leads system to divide by zero, infinite loops, crash failure etc. All smart contract transactions take place within a virtual machine \cite{Dickerson+:ACSC:PODC:2017}. %Virtual machine environment can get rid of the issues of inconsistent read while executing the smart contract transactions sequentially. 
When miner executes the smart contract transactions concurrently on the virtual machine then infinite loop and inconsistent read may occur. So, to ensure the correct concurrent execution, the miner should satisfy the correctness-criterion as opacity \cite{GuerKap:Opacity:PPoPP:2008}.

To achieve better efficiency, sometimes we need to adapt the non-virtual machine environment which necessitates with the safeguard of transactions. As well miner needs to satisfies the correctness-criterion as opacity to ensure the correct concurrent execution of smart contract transactions. %Opacity assures that all the transactions read consistent values including aborted transactions as well. 

%In non-virtual machine environment, any inconsistent read may leads to divide by zero, infinite loops, crash failure of concurrent miner etc. So, the correct concurrent execution by miner should ensures opacity which says all the transactions read consistent values including aborted transactions as well. % The concurrent execution of the \scontract transactions of a block by the validators which although is highly desirable can further complicate the situation. 
\begin{requirement}
	Any history $H_m$ generated by concurrent miner should satisfy opacity.
\end{requirement}
\cmnt{
\begin{proof}
	Here, miner executes the smart contract concurrently with the help of optimistic STM protocols (BTO and MVTO). Internally, BTO and MVTO \cite{Kumar+:MVTO:ICDCN:2014} protocol ensures opacity. So, history $H_m$ generated Concurrent miner satisfies opacity.
\end{proof}
}

%Concurrent miner provides $BG$ to concurrent validators to ensure the correct output by validators. After that concurrent validator apply topological sort on $BG$ and generates a history $H_v$.

%Once a concurrent miner proposes a block, then validator re-executes the same set of transactions concurrently to validate it. But during the concurrent execution, suppose the validator execute two conflicting transactions in a different order from what was executed by the miner. Thus the serialization order of the miner is different from the validator. Then this can result in the validator obtaining a different final state than what was obtained by the miner. Thus the validator may incorrectly reject the block although it is valid. 

Concurrent miner maintains a BG and provides it to concurrent validators which ensures the dependency order among the conflicting transactions. As we discussed in \figref{conmv} of \secref{intro}, if concurrent miner will not maintain the BG then a valid block may get rejected by the concurrent validator. %BG helps to achieve the same final state by concurrent validators as concurrent miner.


\subsection{Requirements of the Concurrent Validator}
The correct concurrent execution by validator should be equivalent to some serial execution. The serial order can be obtained by applying the topological sort on the BG provided by the concurrent miner. BG gives partial order among the transactions while restricting the dependency order same as the concurrent miner. So, validator executes those transactions concurrently which are not having any dependency among them with the help of BG. Validator need not to worry about any concurrency control issues because BG ensures conflicting transactions never execute concurrently.

%For validator, we can use any concurrency control mechanism to execute smart contract transactions concurrently but transactions may abort on conflict and retry. Retrying the conflicting transactions may take time which leads to slow down the performance of concurrent validator. 

\subsection{Requirements of the Block Graph}

As explained above, the miner generates a BG to capture the dependencies between the smart contract transactions which is used by the validator to concurrently execute the transactions again later. The validator executes those transactions concurrently which do not have any path (implying dependency) between them. Thus the execution by the validator is  given by a topological sort on the BG. 

Now it is imperative that the execution history generated by the validator, $H_v$ is `equivalent' to the history generated by the miner, $H_m$. The precise equivalence depends on the STM protocol followed by the miners and validators. If the miner uses Multi-version STM such as MVTO then the equivalence between $H_v$ and $H_m$ is \mvve. In this case, the graph generated by the miner would be multi-version serialization graph \cite[Chap. 5]{WeiVoss:TIS:2002:Morg}. 

On the other hand, if the miner uses single-version STM such as BTO then the equivalence between $H_v$ and $H_m$ is view-equivalence (\vie) which can be approximated by conflict-equivalence (\ce). Hence, in this case, the graph generated by the miner would be conflict graph \cite[Chap. 3]{WeiVoss:TIS:2002:Morg}. 

%In order to improve the efficiency of concurrent validator, we consider $BG$ which allow to execute the transactions concurrently without abort.


%The correct concurrent validator execution obtains a total order among the transactions. The way, we have done the concurrent validators need not to worry about concurrency control issues.

%\subsection{Requirements of the Block Graph}
\cmnt{
Block graph ensures view equivalence between the histories of the concurrent miners and validators. During the concurrent execution of miner using STM\_BTO protocol, conflict graph (same as BG) captures the view equivalence between the histories of the concurrent miners and validators while maintaining single-version corresponding to each data-objects. We can use the STMs for the concurrent execution by validators but aborts will be there. In order to improve the efficiency of concurrent validator, we consider $BG$ which allow to execute the transactions concurrently without abort. Consider the history $H_m$ generated by STM\_BTO protocol and constructs $BG$ in which each committed transaction $T_i$ consider as vertices and edges between them as follows:
\begin{itemize}
\item r-w: If $T_j$ writes $x$ after read by $T_i$ in $H_m$, then there is an edge from $v_i$ to $v_j$. %Note that in order for this to happen, $T_i$ must have committed before $T_j$ and $c_i$ $<_{H_m}$ $w_j(x)$. 
This set of edges are referred to as r-w.
%$T_i$ reads $x$ from $T_k$, after that $T_j$ writes on $x$ data-object then r-w edge will be from $T_i$ to $T_j$.  
\item w-r: If $T_j$ reads $x$ from $T_i$ in $H_m$, then there is an edge from $v_i$ to $v_j$. Note that in order for this to happen, $T_i$ must have committed before $T_j$ and $c_i$ $<_{H_m}$ $r_j(x)$. This set of edges are referred to as w-r.
%If $T_i$ reads $x$ from the value written by $T_j$ then w-r edge will be from $T_i$ to $T_j$. 
\item w-w: If $T_j$ writes to $x$ after written by $T_i$ in $H_m$, then there is an edge from $v_i$ to $v_j$. Note that in order for this to happen, $T_i$ must have committed before $T_j$ and $c_i$ $<_{H_m}$ $w_j(x)$. This set of edges are referred to as w-w.
%If $T_i$ writes into $x$ before written by $T_j$ then w-w edge will be from $T_i$ to $T_j$. 
\item \rt(real-time) edges: If $T_j$ starts after commit of $T_i$ in $H_m$, then there is an edge from $v_i$ to $v_j$. This set of edges are referred to as $\rt(H_m)$.
\end{itemize}

Whereas when we consider the concurrent execution of miner using STM\_MVTO protocol which stores multiple version corresponding to each data-objects, conflict graph can be restrictive. So, we consider Multi-Version Serialization Graph, MVSG $(H_m,\ll)$ for a given version order of history $H_m$ as follows to ensure the multi-version view equivalence between the histories of the concurrent miners $H_m$ and validators $H_v$:
\begin{enumerate}
\item \textit{\rt}(real-time) edges: If $T_i$ commits before $T_j$ starts in $H_m$, then there is an edge from $v_i$ to $v_j$. This set of edges are referred to as $\rt(H_m)$.

\item \textit{\rf}(reads-from) edges: If $T_j$ reads $x$ from $T_i$ who has written on $x$ in $H_m$, then there is an edge from $v_i$ to $v_j$. Note that in order for this to happen, $T_i$ must have committed before $T_j$ and $c_i$ $<_{H_m}$ $r_j(x)$. This set of edges are referred to as $\rf(H_m)$.

\item \textit{\mv}(multi-version) edges: The \mv{} edges capture the multi-version relations and is based on the version order. Consider a successful read \op{} $r_k(x,v)$ and the write \op{} $w_j(x,v)$ belonging to transaction $T_j$ such that $r_k(x,v)$ reads $x$ from $w_j(x,v)$ (it must be noted $T_j$ is a committed transaction and $c_j$ $<_{H_m}$ $r_k$). Consider a committed transaction $T_i$ which writes to $x$, $w_i(x, u)$ where $u \neq v$. Thus the versions created $x_i, x_j$ are related by $\ll$. Then, if $x_i \ll x_j$ we add an edge from $v_i$ to $v_j$. Otherwise ($x_j \ll x_i$), we add an edge from $v_k$ to $v_i$. This set of edges are referred to as $\mv(H_m, \ll)$.
\end{enumerate}

\begin{lemma}
	History $H_m$ generated by MVTO protocol and $H_v$ are multi-version view equivalent.
\end{lemma}
}
